Why Authors Don't Visualize Uncertainty

Clear presentation of uncertainty is an exception rather than rule in media articles, data-driven reports, and consumer applications, despite proposed techniques for communicating sources of uncertainty in data. This work considers, Why do so many visualization authors choose not to visualize uncertainty? I contribute a detailed characterization of practices, associations, and attitudes related to uncertainty communication among visualization authors, derived from the results of surveying 90 authors who regularly create visualizations for others as part of their work, and interviewing thirteen influential visualization designers. My results highlight challenges that authors face and expose assumptions and inconsistencies in beliefs about the role of uncertainty in visualization. In particular, a clear contradiction arises between authors' acknowledgment of the value of depicting uncertainty and the norm of omitting direct depiction of uncertainty. To help explain this contradiction, I present a rhetorical model of uncertainty omission in visualization-based communication. I also adapt a formal statistical model of how viewers judge the strength of a signal in a visualization to visualization-based communication, to argue that uncertainty communication necessarily reduces degrees of freedom in viewers' statistical inferences. I conclude with recommendations for how visualization research on uncertainty communication could better serve practitioners' current needs and values while deepening understanding of assumptions that reinforce uncertainty omission.

==> notes.tex <==
signal detection - have the rule and the probability

\jessica{hindsight bias} Outcome knowledge increases predicted likelihood of events 


\textbf{what about stakes - stakes matter - Cox}

FE: ``I think about the difference between a visualization meant to learn from and a visualization meant to take action on. They're different things with a totally different process. I think about that all the time. ''

\textbf{On Decisions and Actions}: 
Within research on uncertainty communication, scholars have distinguished between different types of decisions, and recommended different strategies for uncertainty assessment and communication based on these decision types~\cite{fischhoff2014communicating}. The goal of a message may be to provide a categorical signal (e.g., should you evacuate?), to help the user choose among fixed options (e.g., should you invest in this treatment?), or to create new options (e.g., developing policy around a new technology). 

People will judge science's value by the apparent wisdom of recommendations from it. Do calls to action seem to lead to saving lives etc or needless shelter taking, surgery etc? These evals should depend on uncertainty in the science and appropriateenss of hte rule translating into into a recommendations. In retropsect, such evals can be colored by outcoem bais, arising w hen decisions are judged by their outcoems rather than by their wisdom, and by hindsight bias, arising when people exaggerate how well those outcomes could have been foreseen. 

Even when DMs resist such biases, they can judge science fairly only if they can see its evidence through the filter of the recommendations.  With a single event, they can't disentangle the evidence and decision rule on their own but must be told how this advice was reached.

With multiple events, decision makers can infer the quality of the science and the decision rule from the pattern of decisions and outcomes. As formalized by signal detection theory, quality is represented by d prime )(how well experts can discriminate among states of hte world) and decision rules are represented buy beta )thje tradeoffs made among possible outcomes) - 

signal detection - estimation is harder when they have to infer both parameters, compared to when they know one and must estimate the other. Experts can communicate the rules for example. 

In decision science, one way to determine how much people need to know about the likelihood of possible states of the world is to query whether there are any plausible states under which one's action would differ~\cite{}. For example, one could ask ``would any plausible value for a predicted vote choice for candidate A based on survey data cause you to change your plan to vote and for whom?'' If the answer is no, then one could argue that uncertainty information has no clear purpose in that communication scenario. If a visualization author believes that their work communicates data that is immaterial to any real world actions (\textit{criterion 1}), then defaulting to not presenting uncertainty may be reasonable. 


Fischoff and Davis: 
The information that needs to be communicated depends on the decisions that people face. Are they (i) looking for
a signal (e.g., whether to evacuate before a hurricane), (ii) choosing among fixed options (e.g., which medical treatment is best), or
(iii) learning to create options (e.g., how to regulate nanotechnology)? We examine these three classes of decisions in terms of how
to characterize, assess, and convey the uncertainties relevant to
each. 


\jessica{move}:
And yet, despite the lack of consensus in attitudes as a whole, commonalities were 
apparent in how influencers perceived certain rhetorical aspects of uncertainty information, and where online survey respondents appeared to perceive the extremes in attitudes. Two statements in particular, both of which stated strong views about the appropriateness of uncertainty information, produced a remarkable degree of consensus among authors. Authors consistently agreed that ``uncertainty information should be presented when it calls into question the main message or pattern shown in the visualization'' (Figure~\ref{fig: }; mean: 4.6, sd: 0.65) and disagreed that ``uncertainty information is only appropriate for data experts'' (Figure~\ref{fig: } mean: 1.8, sd: 0.88). 



One influencer described how ``in theory, I should have a lot of uncertainty. I'm working with very hardcore statisticians and machine learning experts and scientists, and yet i don't explicitly include uncertainty in my visualizations ever. It was actually quite interesting, after your prompt, thinking about why.''


\subsubsection{Uncertainty as Responsibility}
Among those interviewees, survey respondents, and focus group participants who believed uncertainty representation should be more common, multiple described uncertainty as a responsibility assumed by an author in presenting data to others. Focus group participants argued for the importance of transparency in media presentations of data, suggesting that omitting uncertainty was misleading or even lying. 
An influencer, in describing how readers' trust in the accuracy of visualized data was often a priori and orthogonal to uncertainty presentation, proposed that ``if you have trust, you probably should [show uncertainty], because you can afford that space.''

\subsubsection{Uncertainty as Education (+)}
Several influencers who were symptathetic to uncertainty communication ideals described an educational potential they perceived in commonplace uncertainty representation. An influencer who is a graphics editor at a news publication described wanting to show uncertainty more often to help her audiences become accustomed to what scientific measurement is like: ``I don't always give that [quantifiable uncertainty] the attention it deserves. That's where I want to start to get better in terms of representing -- I feel like once readers start to understand that there's uncertainty inherent in a lot of these things, it's still significant. To get used to the idea that this can be very rigorous and still have a range of uncertainty, that's where I feel like I need to get better at not just saying, `Well, we'll just show these data points'
Focus group participants similarly argued for uncertainty presentation as a default because ``otherwise people won't get better at realizing nuances in data.''
Another graphics editor who voiced a desire for more commonplace uncertainty representation replied sarcastically ``oh, they don't care'' when asked about 
norms and ideals around uncertainty in her organization. 
Another influencer thought that \textit{not} presenting uncertainty in favor of simplification cultivated an undesirable impatience in visualization audiences.


An influencer, in describing how readers' trust in the accuracy of visualized data was often a priori and orthogonal to uncertainty presentation, proposed that ``if you have trust, you probably should [show uncertainty], because you can afford that space.''

\textbf{as if optimization}
The omission of uncertainty as an attempt to bring about great coordination was recently addressed by Manski~\cite{manski2018lure}, who uses the term ``as-if optimization'' to refer to the reporting of only a point (maximum likelihood) estimate. Arguments for coordination may refer to how uncertainty can lead to a greater heterogeneity in interpretations relative to a single point.  
Though not explicitly descriptive of a coordination benefit, one influencer quoted another author's explanation of why an audience at large desires a single best estimate without uncertainty to function: 
``We don't quantify [the uncertainty] because what matters to the audience is knowing that scientists are doing their best with what they have and that this is the best information we have right now. This is what people want in order to make decisions or take actions.'' 



%This formalization is useful for understanding visualization-based inferences in that it can account for signals of varying complexity. While in the simplest case the visualization might display only a single scalar value (e.g., a difference between the means of two sets of measurements, a single measurement or statistic), defining the test statistic as a vector means that the entire visualization can function as the test statistic. The second is that the formalization defines the ``truth'' of a signal relative to an observer. There is nothing in this definition that prevents the idea of different authors having different critical values for . 



implicit in the fact that authors engage in the visualization process to validate and tune the signal is an assumption that viewers also engage in a process of signal validation when they view the visualization. In other words, each viewer separately produces a test statistic $T(y)$.  






%As a result, a logical fallacy in any single tenet invalidates the system. Below I draw on theories of inference from linguistic philosophy and graphical statistical inference to expose fallacies. 

%\jessica{A logical fallacy with the model stems from the fact that it implies that visualizations function in two different ways for authors and users. More precisely, the model implies that by default, a signal is judged to be true in a binary way by viewers but that authors perceive signals on a spectrum. 
%Below, I present a common sense ``proof'' of this fallacy. To reduce ambiguity in the argument, which is statistical in nature, I formalize key operations and trade-offs. %My goal in this formalization is not to propose a definitive quantitative model but rather, in the vein of van Wijk's ``The Value of Visualization''~\cite{vanwijk} to give a sense of quantification.}
%I believe that attempting formal descriptive models is an important step in aligning visualization research with practice. 
%hat can nonetheless be useful for identifying 
%The gist of the proof is that for visualization to function as a means of conveying signal, users cannot be unsusceptible to uncertainty. Users will necessarily arrive at subjective estimates of the probability that signals conveyed by visualizations are true. 

%\subsection{Informal Proof}
The function of a visualization in the rhetorical model is to convey a signal. 

.  are compared to data replicated under some model. In standard significance testing, this model is represented by the null hypothesis. 

The reference distribution corresponds to a model for data generation. 



 


, however, to be effective enough to present to others in a visualization a signal must pass a threshold.


A visualization without a signal is possible but these visualizations are not shown.  
A signal must therefore 

(Even if other statistical means are used, authors suggested that the visualization step is still important for confirming that this signal exists.)  Hence, the visualization is a test statistic for the author. 
If the author had a signal without any analytical process behind it whatsoever, for example if they were handed a signal in a dream, and created a visualization of this signal, it would seem obvious that the signal 



, but this is not possible under the assumption that visualizations []

------
Assume the signal has some probability of being` invalid, that is, produced by coincidence, and that an omniscient statistician has calculated this 



$p_{sig}$

what determines perceived $p_{sig}$?

One possibility is that it is 1 bc trust is a priori and when ppl don't trust source this seems to 



Well, we know that showing uncertainty reduces the average perceived probability $mean(p_{sig})$


 





----
Model suggests that its binary when uncertainty is not shown. people don't question. 

This implies that the test statistic produces a p value of 0 for the core signal. 



But for people to not question at all would mean that their prior on the probability that its true is 1. If this is the case, then the vis pattern would be interpreted as precise to the max. 

If they interpret things this way, then the author would not need to worry about signal strength in the design process. That process assumes that the apparent signal can be altered by the design. For the design process to happen, the author has to assume that whatever strength it appears to have them in the visualization is analogous to the strength it will appear to have for the user.






------

The process of eda/whatever is what identifies the signal. Having a signal without the process would imply a lie.

That trust in source alone determines whether or not someone will get the message implies binary state space for interpretations - either get it or don't (showing uncertainty means they don't get it for the obfuscation reasons above)

this implies that the viewer can't look at a vis and get a sense of the probability that its right , or maybe only in the trust case
---------

Another fallacy derives from statistical inference. 


\subsubsection{CX Fallacy:}
Combining Tenet 1 and 2 implies that the signal in a visualization is analogous to a magnitude rather than a test statistic.





%Having a relatively minimal set of tenets become useful for reasoning about the potential problems with a norm of uncertainty omission. Here, problems could be defined by appealing to various bases for truth. While a moral responsibility for presenting uncertainty has been argued elsewhere~\cite{fischhoff2012communicating} and might find support in some influencers and authors I surveyed, I propose that a more convincing argument for problems with the current model is one that exposes logical flaws in how it defines meaning. %786509If the model [explain]
%I therefore demonstrate logical gaps in the model by appealing to three different theories of inference with applications to uncertainty: philosophy of linguistics, graphical statistical inference, and rational decision-making.  

\subsubsection{Trust Fallacy:}
graphical statistical inference:
A first logical problem stems with the implication of a dynamic in which messages are either trusted on faith or not trusted at all. This dynamic implies that the state space of interpretations that are possible from a communication-oriented visualization may be binary: a reader either believes the pattern they are seen, or they do not. 
But this contradicts how we identify a pattern to begin with - we have to judge a visual thing we see relative to some reference and that tells us if it is in fact a thing. Our confidence is based on much more of a thing it seemed to be than the other things.  that a visualization could convey a signal in a way that sidesteps this visual inference process would seem contradicted by the importance of the eda process to produce the signals that are shown to begin with. If authors are presenting patterns that they observed rather than made up, then some analogous thing must be happening for the viewer. That thing is by definition not a binary yes no 

If we don't visualize uncertaitntyt, what is the pattern judged against? 


A lack of trust in the author of a visualization was also cited as a critical roadblock in the conveyance of the message: ``It actually takes quite a lot to look at something from a source you're not really sure of, but you're aware you're unsure of that source, and it gives you new information that makes you question something you've already thought. All of that, that's a lot. A lot of people don't do that. They'll even stop at that early stage, ``This is from a source I don't trust. I'm not going to listen to it.''  Several other influencers and survey respondents similarly alluded to trust as all or nothing. %, for example: ``Data is often ambiguous and can still be useful, data is presented too often as hard science and we need to communicate in a way that does not encourage a binary approach but is still responsible.''


\jessica{move} Adding complexity by presenting uncertainty poses the risk of losing the viewer's attention, or making them doubt that you as author can be trusted. The ways in which authors referred to trying to keep users interested suggests that rather than estimate uncertainty, the conventional uncertainty describing how a pattern or estimate might take any value from a range, authors are concerned with what might be called \textit{interpretation uncertainty}, referring to uncertainty in the probability that a user believes the message. 
If maximizing the number of viewers who adopt the signal is the goal of visualization, then 



A second logical problem with the model relates to how faith in process appears to be used to rationalize omission of uncertainty among many authors. Wittgenstein's linguistic philosophy argues that the meaning of a statement (word) is based entirely in the role it plays in a ``language game.''  \jessica{explain how if the statements only get their truth value within the system, then it is impossible to s}


%\textbf{as if optimization}
%FE quoting ``OF course it's not perfect information. It's at least the best we have.'' That is what people want in order to make decisions or take actions. they want to know that at least they're sitting on the best. 
\textbf{state space binary approach}: 


\jessica{move: } ``uncertainty (e.g., error of mean) very low \& error bars added nothing''

, concerning ``the grounds of knowledge 
of knowledge especially with reference to its limits and validity''\yeaseul{}~\cite{merriam}.
Authors 
Epistemology refers to 
the distinction between justified belief and opinion.


\subsection{Estimate Uncertainty vs Interpretation Uncertainty}
The strongest rationale that emerged concerned a fundamental questioning of the rhetorical function of uncertainty. Authors [describe]


`There's always a creeping temptation, not just from the client to say as much as possible, but also myself. I get caught up in the mood of a subject and think, ``That's interesting. That's interesting.' Again, you have to step back and think you can't serve everyone's potential appetite. That's why you have to realize that you will ultimately have to frustrate some potential audiences.'

``It's a constant battle to get bums on seats, but also then to make it worthwhile for that bum being on the seat.''

`` It's an undertaking from just the amount of work involved., but also for -- you're analyzing your audience. Sometimes the editor is going to say, `We're going to lose views on this,' so they'll want to. '' FE



%\subsection{Uncertainty in Language Games}
\jessica{wittgenstein} Language is a game, or a continuous play of meaning governed by various guidelines which may be understood implicitly but remain unstated. 
While the definitive meaning of a statement resists determination, due to variation in private interpretations, the indefinite aspect finds its complement in the very real actions that result
from communication.
The rules of the game need not be interpreted identically by the players for the game to be successful. They must only allow for further action
and communication.


On the one hand, as common ground is established utterances in a language can become more efficient. (Wittgenstein - `that' the meaning of the word is its use, meaning we don't have to waste words if the same function can be acheived with fewer)


As seam: When uncertainty is communicated, interpretation hovers between ``know'' and ``don't know,'' threatening to expose a system which, once visible, must be reconstructed for the receiver all the way down. 

A logical fallacy that people agree should present it if the pattern is questionable
-what determines what is questionable? 
-process


The omission of uncertainty is equivalent to a statement 'I know' or 'I am certain that'.
[problems]

at the extreme, we could liken the exploratory data analysis process to a calculation - governed by rule(s)
but is there a rule describing when a mistake is impossible?

proposition that many journalists return to - we vetted it, would have caught it if fake - faith in process
but because the proposition itself is senseless without the process, should
instead focus these statements on what it looks like when a mistake is made
In other words, to say 'We know this is right' is to instruct on the process and what labels we can apply when we have used the process

most would agree that the process can be likened to a statement in a statistical language.
sure its 'significant' - sure its not due to chance -- about inference - procedures that are guaranteed under hypothetical conditions where we know the population value. 
But more often than not we admit we can't know the population value because its outside the realm of reasonable measurement.
So our statements about the process are best considered statements of instruction and faith.

What is interesting is how we use the process; the meaning of a word is its use.

\jessica{The truth of my statements is the test of my understanding of these statements 81. That is to say,that if I make certain false statements, it becomes uncertain whether I understand them.  82.  What counts as an adequate test of a statement belongs to logic. It belongs to the description of the language-game}

Show that authors operate as though there is an implicit assumption that when uncertainty is omitted, confidence will be at least as high as actual and more people will get the message. 
(ie get the strongest signal across)

When its shown, confidence is more likely to be calibrated across those who perceive the message. 
(ie get the most accurate signal across)





%``… imagine having to sketch a sharply defined picture ‘corresponding’ to a blurred one. In the latter there is a blurred red rectangle: for it you put down a sharply defined one. Of course—several such sharply defined rectangles can be drawn to correspond to the indefinite one.—But if the colours in the original merge without a hint of any outline won’t it become a hopeless task to draw a sharp picture corresponding to the blurred one? Won’t you then have to say: “Here I might just as well draw a circle or heart as a rectangle, for all the colours merge. Anything—and nothing—is right. (36)




39. \textit{This} is how calculation is done; in such circumstances a calculation is \textit{treated} as absolutely reliable, as certainly correct.
40. Upon 'I know that here is my hand' there may follow the question 'How do you know?' and the answer to that presupposes that \textit{this} can be known in \textit{that} way. So, instead of 'I know that here is my hand', one might say 'Here is my hand' and then add \textit{how} one knows.

63. If we imagine the facts otherwise than as they are, certain language-games lose some of their importance, while others become important. And in this way there is an alteration--a gradual one--in the use of the vocabulary of a language.
79. That I am a man and not a woman can be verified, but if I were to say I was a woman, and then tried to explain the error by saying I hadn't checked the statement, the explanation would not be accepted.
\jessica{The truth of the statement 'uncertainty doesn't need to be presented' is the test of my understanding of that statement. If it were to be shown that I made a false statement, it would become uncertain whether I can in fact tell when uncertainty shouldn't be presented. In fact if I really want to make a strong statement, I should show uncertainty, because they would convey that I am confident in my `message' and in my implicit statement 'uncertainty doesn't need to be presented' - this doesnt make sense??? 
If authors are worried about their own ability to adequate understand uncertainty, hiding may help in cases where their 'message' is not found to be wrong. In a case where it is found to be wrong,   } 
80. The \textit{truth} of my statements is the test of my \textit{understanding} of these statements
81. That is to say, that if I make certain false statements, it becomes uncertain whether I understand them. 
82. What counts as an adequate test of a statement belongs to logic. It belongs to the description of the language-game. 

[maybe talk about norms - much of what we believe is inherited . to what extent is the appeal to the process dependent on the norm of not presenting uncertainty? 
the propositions describing this world-picture might be part of a kind of mythology. And their role is like that of the rules of a game; and the game can be learned purely practically, without learning any explicit rules]
94. But I did not get my picture of the world by satisfying myself of its correctness; nor do I have it because I am satisfied of its correctness. No, it is the inhereted background against which I distinguish between true and false. 

%\jessica{The system, which encompasses all of the ways in which interpret statistical inference procedures to convey some facts but not others, is the substrate for all of our arguments about what is true or not true. There is no outside 'fact' or 'not fact'. Our system tells us what is and what is not a reasonable thing to doubt. If we perceive that doubting something would open up many questions that we can not answer (e.g., how could such a large difference arise by chance? why would an author with a reputation for good work present this if they did not know it was true?), we believe it more reasonable to accept it as true (the omission of uncertainty). If someone were to look at a presentation of data that omitted uncertainty and say 'This is wrong. I don't know how its wrong, but I know that it is wrong and there are some things that we still can't explain' one would feel very intellectually distant from whoever said that.
%We are in a place with uncertainty visualization where to some it seems absurd for someone to say 'we should always present uncertainty' and to others  .And yet, the omission of uncertainty is in no way a guarantee}




105. All testing, all confirmation and disconfirmation of a hypothesis takes place already within a system. And this system is not a more or less arbitrary and doubtful point of departure for all of our arguments; no, it belongs to the essence of what we call an argument. The system is not so much the point of departure, as the element in which arguments have their life.

108. If we are thinking within our system, then it is certain that no one has ever been on the moon. Not merely is nothing of the sort ever seriously reported to us by reasonable people, but our whole system of physics forbids us to believe it. For this demands answers to the questions ``How did he overcome the force of gravity?'' ''how could he live without an atmosphere?'' and a thousand others which could not be answered. But suppose that instead of all these answers we met the reply: ''We don't know \textit{how} one gets to the moon, but those who get there know at once that they are there; and even you can't explain everything.'' We should feel ourselves very intellectually distant from someone who said this.

What is the test that is being done? 

121. Can one say, where there is no doubt there is no knowledge either?
122. Doesn't one need grounds for doubt. 
123. Wherever I look, I find no grounds for doubting that...
(when a challenge is not presented or we see no evidence that we could be wrong then we don't really consider it reasonable to doubt)
124. I want to say: We use judgments as principles of judgment. 
(we see no reason to doubt as we prepare things (a judgment) therefore we have grounds for being certain

130.  But isn't it experience that teaches us to judge like \textit{this}, that its to say, that it is correct to judge like this? But how does experience \textit{teach} us, then? \textit{We} may derive it from experience, but experience does not direct us to derive anything from experience. If it is the \textit{ground} of our judging like this, and not just the cause, still we do not have a ground for seeing this in turn as a ground.
131. No, experience is not the ground fro our game of judging. Nor is its outstanding success.
(in the past, our process has been a good guide - we have empirical evidence that what we are doing is good. But this is our choice to see the acceptance of what we've reported in the past or fact that its turned out to be predictive of reality. We may have reason to want to see it that way since it saves us work worry complication now. Its a judgment, there is nothing that says 'this is the right way to do things')

From Wittgenstein~\cite{wittgenstein1969}:
What we can ask is whether it can make sense to doubt it. 
Whether a proposition can turn out false after all depends on what I make count as determinants of that proposition. 
The difference between the concept of 'knowing' and the ocncept of 'being certain' isn't of any great importance at all, except where 'I know' is meant to mean: I can't be wrong.
In a law-court for example, 'I am certain' could replace 'I know' in every piece of testimony. We might even imagine it being forbidden to say 'I know' there.
11. We just do not see how very specialized the use of 'I know' is.
12. For 'I know' seems to describe a state of affairs which guarantees what is known, guarantees it as a fact.
13. For it is not as though the proposition 'It is so' could be inferred from someone else's utterance: 'I know it is so'.
14. That he does know takes some showing.
15. It needs to be shown that no mistake is possible. It needs to be objectively established that I am not making a mistake in assuming 'I know' (i.e., that I have not made a mistake). 
16. 'If I know something, then I also know that I know it' amounts to: 'I know that' means 'I am incapable of being wrong about that.' But whether I am so needs to be established objectively.

\subsection{Uncertainty in Graphical Statistical Inference}



%elsewhere: ``This is one of the big differences between communication vis and analysis vis and really flipping between those two. A lot of the rules we've constructed for vsiualziation in terms of those first-time rules that you leanr when you start doing data vis, are really formed around ocmmunication, I mean, that makes a lot of sense. Many people are there ... A lot of people do exploratory, but they just aroen't thinking about what they're doing when they're in the process. When you're doing communication vis, it's much more about how do you make sure that the person doesn't read something into it that isn't there? In analysis vis, the bigger risk is overlooking something important.''


\subsection{Uncertainty in Rational Decision-Making}

utility functions are used to represent preference relationship

van Wijk's value of visualization: ``Nevertheless, we should try to measure or estimate $W(\delta K)$, if we want to assess the value of visualization, especially because it is the only term in the model for $F$ with a positive sign. An operational approach is to consider the use of visualization as an element in problem solving. The user has a problem, he must decide which action to take, and to make that decision he needs information. The visualization should enable him to extract the relevant information from the data.'' \jessica{related to underspecified decisions}


change in knowledge $\frac{dK}{dy}=P(I,K)$ where P is particular properties of perception and cognition of user

current knowledge K(tT) follows from integration over time:
$K(t) = K_{0} + \int_{0}^{t} P(I, K, t)dt$

$K_{0}$ is initial knowledge

An important aspect is interactive exploration, E(K). user may decide to adapt the specification of vis base on his current knowledge in order to explore data furtherrr
$\frac{dS}{dt}=E(K)$ hence the current spec S(t) follows from integration over time:
$S(t) = S_{0} + \int_{0}^{t} E(K) dt$ where $S_{0}$ is initial spec

econ model - 
In van Wijk's model we have total costs of a vis 
\[ C=C_{i} + nC_{u} + nmC_{s} + nmkC_{e} \]
where $C_{i}$ is initial development cost, $C_{u}$ is initial costs per user (selection and acquisition of V, how to use it, tailoring to needs - V is a vis system), $C_{s}$ is initial costs per session, $C_{e}$ is perception and exploration costs.

Return on these investments consists of hte value W(change in K) of he acquirred knowledge change in K = K(T) = K(0) per session multiplied by total number of sessions:
$G=nmW(change in K)$
and hence for the total porfit F=G-C we find
$F-nm(W(change in K) - C_{s} - kC_{e}) - C_{i} - nC_{u}$
provides a recipe to decide on the value of a vis method. Positive are high values forrn , m , W(change in K) and low values for all the Cs and k. Or in other words, a great vis is used by many who use it routinely to obtain highly valuable knowledge without having to spend time and money on hardware, software, and effort. 

\textbf{Manski formulation}: Rationale -- bounded rationality -- people have limitations, need to approximate so not showing it simplifies decision making - Manski calls it as-if optimization

Choice among options where value of some options depends on the state of nature
S=State space - list of stats of nature S includes [main pattern T, main pattern F]

C=choice set - [gather more info, act]
A first step would be to ask whether one of these dominates the others, specifically whether there is d in C such that w(d,s) greater than or equal to w(c,s) for all s in S and w(d,s) > w(c,s) for some s. To check we can ask, can we imagine a state whether the utility of gathering more info is less than simply acting? Rationales (X,Y,Z) reported above may suggest yes, given the following reasoning: when the core message of the visualization is true then the marginal utility of presenting uncertainty 


those who don't - if DM asserts knowledge of objective probability distribution on state space P, this is rational expectations and they maximize expected utility is 

\[
  \max_{c \in D} \int w(c,s)dP 
\]




\textbf{Uncertainty on demand}
Mentioned by several interviewees (Cox, Kirk, ?) 
Dragicevic - Signalling transparency and research integrity 
Writing these things will remain hard
many suggest things at 2 levels - those who want to explore it/see uncertainty
those who don't - if DM asserts knowledge of objective probability distribution on state space P, this is rational expectations and they maximize expected utility is 

\[
  \max_{c \in D} \int w(c,s)dP 
\]
Uncertainty that is hidden until demanded introduces heterogeneity in the form of some subset of people having 
\[
  \max_{c \in D} \int w(c,s)d\pi_{vis} 
\]
where $pi_{error}$ is a subjective distribution on the state space informed by the uncertainty presentation, and others having either the first one or more realistically:
\[
  \max_{c \in D} \int w(c,s)d\pi_{est} 
\]
where $\pi_{est}$ is an estimated subjective distribution on the state space. 
In a state space consisting of only the two states `The visualized statement is true', `The visualized statement is false', for any individual $\pi_{vis}$ (or conversely $\pi_{est}$) can be summarized by a single probability $P($'The visualized statement is true'$)$.  If we treat  $\Pi_{vis}$ and $\Pi_{est}$ as random variables then $Var(\Pi_{est}) > Var(\Pi_{vis})$ as $Var(\Pi_{est})$ wherever the average error an individual faces in inferring $\pi_{vis}$ is smaller than what they would face in inferring $\pi_{est}$





